Robust and Verifiable MPC with Applications to Linear Machine Learning Inference

In this work, we present an efficient secure multi-party computation MPC protocol that provides strong security guarantees in settings with dishonest majority of participants who may behave arbitrarily. Unlike the popular MPC implementation known as SPDZ [Crypto '12], which only ensures security with abort, our protocol achieves both complete identifiability and robustness. With complete identifiability, honest parties can detect and unanimously agree on the identity of any malicious party. Robustness allows the protocol to continue with the computation without requiring a restart, even when malicious behavior is detected. Additionally, our approach addresses the performance limitations observed in the protocol by Cunningham et al. [ICITS '17], which, while achieving complete identifiability, is hindered by the costly exponentiation operations required by the choice of commitment scheme. Our protocol is based on the approach by Rivinius et al. [S&P '22], utilizing lattice-based commitment for better efficiency. We achieved robustness with the help of a semi-honest trusted third party. We benchmark our robust protocol, showing the efficient recovery from parties' malicious behavior. Finally, we benchmark our protocol on a ML-as-a-service scenario, wherein clients off-load the desired computation to the servers, and verify the computation result. We benchmark on linear ML inference, running on various datasets. While our efficiency is slightly lower compared to SPDZ's, we offer stronger security properties that provide distinct advantages.

==> macros.tex <==
\RequirePackage{xfrac}
\RequirePackage{amsmath}
\RequirePackage{amsopn}
\RequirePackage{ifthen}
\RequirePackage{xcolor}
\RequirePackage{xspace}
\RequirePackage{xparse}
\RequirePackage{algpseudocode}
%\RequirePackage{amsthm} 
\RequirePackage{amssymb}%need this for \blacksquare
\RequirePackage{tikz}

\renewcommand{\paragraph}[1]{\medskip\noindent{\bf #1}}

\newcommand{\ignore}[1]{}  %Ignores inside when typesetting

% \usepackage{amsmath}
% DEFEQ
\newcommand*{\defeq}{\stackrel{\text{def}}{=}}

%\newenvironment{claim}[1]{\par\noindent\underline{Claim:}\space#1}{}
\newenvironment{claimproof}[1]{\par\noindent\underline{Proof:}\space#1}{\hfill $\blacksquare$}
\newenvironment{theoremproof}[1]{\par\noindent\underline{Proof:}\space#1}{\hfill $\blacksquare$}
% AUTHORS' NOTES <<<
\def\showauthnotes{1}
\ifthenelse{\showauthnotes=1}
{
\newcommand{\authnote}[2]{{ \footnotesize \bf{[#1: #2]~}}}
%\newcommand{\authnote}[2]{{ \tt {[#1: #2]~}}}
}
{ \newcommand{\authnote}[2]{} }

\newcommand{\juan}[1]{{\color{blue}\authnote{Juan}{#1}}}
\newcommand{\jason}[1]{{\color{red}\authnote{Jason}{#1}}}


\newcommand*{\QED}{\null\nobreak\hfill\ensuremath{\square}}%
\newenvironment{nffunc}[3][Functionality]{
\begin{center}
  \begin{tabular}{|ll|}
    \hline
    \hspace{.3ex}
    \begin{minipage}{.98\linewidth}
      \vspace{0.5ex}
      {\begin{center}{\bf #1} #2 \end{center}}
      \vspace{-2ex}#3
      \begin{itemize}
        \vspace{-1ex}
        }{
      \end{itemize}
      \vspace{-1ex}
    \end{minipage}& \\
    \hline
  \end{tabular}
\end{center}
}


\newenvironment{vnffunc}[3][]{
\begin{center}
   \begin{tabular}{|ll|}\hline
     \hspace{.3ex}\begin{minipage}{.92\linewidth}\vspace{0.5ex}
       {\begin{center}{\bf Functionality} #2 \end{center}}\vspace{-2ex}#3 %\begin{itemize}%\setlength{\itemsep}{0mm} \setlength{\parskip}{0pt}
% \setlength{\parsep}{0pt}
%\vspace{1ex}%\vspace{-3ex}
       }{%
       %\end{itemize}
       %\vspace{-1ex}
       \smallskip
     \end{minipage}& \\
     \hline
   \end{tabular}
   \end{center}
}




\newenvironment{nff}[3][]{
\begin{center}
   \begin{tabular}{|ll|}\hline
     \hspace{.3ex}\begin{minipage}{.92\linewidth}\vspace{0.5ex}
       {\begin{center}{} #2 \end{center}}\vspace{-2ex}#3 \begin{itemize}%\setlength{\itemsep}{0mm} \setlength{\parskip}{0pt}
% \setlength{\parsep}{0pt}
\vspace{-1ex}%\vspace{-3ex}
       }{%
       \end{itemize}
       \vspace{-1ex}
       \smallskip
     \end{minipage}& \\
     \hline
   \end{tabular}
   \end{center}
}



\newenvironment{nfprot}[3][]{
\begin{center}\small
  \begin{tabular}{|ll|}\hline
        \hspace{.3ex}\begin{minipage}{.95\linewidth}\vspace{0.5ex}
          {\begin{center}{\bf Protocol} #2 \end{center}}\vspace{-2ex}#3 % \begin{enumerate}\setlength{\itemsep}{2mm} \setlength{\parskip}{0pt}
% \setlength{\parsep}{0pt}
%\vspace{-1ex}%\vspace{-3ex}
          }{%
%          \end{enumerate}
          \vspace{-1ex}
          \smallskip
        \end{minipage}& \\
        \hline
  \end{tabular}
  \end{center}    \vspace{-5ex}
}

\newenvironment{inbox}%
{
    \begin{tabular}{|ll|}\hline\hspace{.3ex}
    \begin{minipage}{.85\linewidth}\vspace{0.5ex}
}%
{
    \vspace{0.5ex}
    \end{minipage}& \\
    \hline
    \end{tabular}
}

\newenvironment{protocol}[3][{\bf Protocol}]{
  \begin{center}
    \begin{tabular}{|ll|}
      \hline
      \hspace{.3ex}
      \begin{minipage}{.95\linewidth}\vspace{.5ex}
        {\begin{flushleft}{\bf #1} #2\end{flushleft}}
        \vspace{-2ex}#3
        \begin{enumerate}
          \vspace{-1ex}
          }{
        \end{enumerate}
        \vspace{-1ex}
      \end{minipage}& \\
      \hline
    \end{tabular}
  \end{center}
}

\iffalse
\newenvironment{IdealFunction}[3][]{
  \begin{center}
    \begin{tabular}{|ll|}
      \hline
      \hspace{.3ex}
      \begin{minipage}{.95\linewidth}\vspace{.5ex}
        {\begin{center}{\bf #1} Functionality #2\end{center}}
        \vspace{-2ex}#3
        \begin{enumerate}
          \vspace{-1ex}
          }{
        \end{enumerate}
        \vspace{-1ex}
      \end{minipage}& \\
      \hline
    \end{tabular}
  \end{center}
}
\fi
\iffalse
\newenvironment{IdealFunction}[3][]{%
  \begin{center}
    \begin{tabular}{|p{\linewidth}|}
      \hline
      \vspace{-1ex}
      \begin{center}
        {\bfseries #1} Functionality #2
      \end{center}
      \vspace{-2ex}
      #3
      \vspace{1ex}
      \begin{enumerate}[leftmargin=2em, label=\arabic*., itemsep=0.5ex, parsep=0pt]
}{%
      \end{enumerate}
      \vspace{-1ex} \\ \hline
    \end{tabular}
  \end{center}
}
\fi

\newenvironment{Simulator}[3][\begin{center} \end{center}]{
  \begin{center}
    \begin{tabular}{|ll|}
      \hline
      %\hspace{.3ex}
      \begin{minipage}{.95\linewidth}\vspace{.5ex}
        {\begin{center}{\bf #1} Simulator #2\end{center}}
        \vspace{-2ex}#3
        \begin{enumerate}
          \vspace{-1ex}
          }{
        \end{enumerate}
        \vspace{-1ex}
      \end{minipage}& \\
      \hline
    \end{tabular}
  \end{center}
}
%\makeatletter
%\newtheorem*{rep@theorem}{\rep@title}
%\newcommand{\newreptheorem}[2]{%
%\newenvironment{rep#1}[1]{%
% \def\rep@title{#2 \ref{##1}}%
% \begin{rep@theorem}}%
% {\end{rep@theorem}}}
%\makeatother

% The set of all possible views does not depend on the environment and simulator, but it is easy to convert this back by just changing the command:
%\newcommand{\Fview}{\iview^{\frel}_{\frel,\Sim,\env}}
\newcommand{\Fview}{\iview_{\frel}}
\newcommand{\Zview}{\iview_{\env}}

\def\mc{\mathcal}

\newcommand{\adv}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\dum}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\dist}{\ensuremath{\mathcal{D}}\xspace}
%\newcommand{\abortAdv}{\ensuremath{\adv_\dagger}\xspace}
\newcommand{\abortAdv}{\ensuremath{\adv_{\rm gen}}\xspace}
\newcommand{\algo}{\mathcal{B}}
\newcommand{\env}{\ensuremath{\mathcal{Z}}\xspace}
%\newcommand{\func}[1][\relax]{\ensuremath{\mathcal{F}_{\textsc{#1}}}\xspace}
\newcommand{\wrap}[1][\relax]{\ensuremath{\mathcal{W}_{\textsc{#1}}}\xspace}
\newcommand{\comp}{\mathcal{C}}
%\newcommand{\fsfe}{\func{SFE}}
\newcommand{\PH}{\mathcal{H}}
\newcommand{\D}{\ensuremath{\mathsf{D}}\xspace}
\newcommand{\M}{\ensuremath{\mathcal{M}}\xspace}
\newcommand{\Y}{\ensuremath{\mathcal{Y}}\xspace}
\renewcommand{\sim}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\nt}[1]{\ensuremath{[#1]}\xspace}
%\newcommand{\exec}{\ensuremath{{\sf Exec}}\xspace}
\newcommand{\exec}{\ensuremath{\textsc{exec}}\xspace}
\newcommand{\ideal}{\ensuremath{\textsc{ideal}}\xspace}
\newcommand{\view}{\ensuremath{\textsc{view}}\xspace}
\newcommand{\indist}[1][\relax]{\ensuremath{\overset {#1}{\approx}}}
\newcommand{\negeq}{\ensuremath{\mathrel{\accentset{\ \mathsf{negl}}{\mathop\approx}}}}
\newcommand{\neglgeq}{\mathrel{\accentset{\ \mathsf{negl}}{\mathop\geq}}}
%\newcommand{\neglleq}{\mathrel{\accentset{\ \mathsf{negl}}{\mathop\leq}}}
\newcommand{\neglle}{<}
\newcommand{\neglge}{>}

%%%% Such that we can easily switch between greedy and rational
\newcommand{\rational}{rational\xspace}
\newcommand{\Rational}{Rational\xspace}

\newcommand{\SPDZ}{\ensuremath{\Pi_{\textrm{SPDZ}}}}
\newcommand{\RVSPDZ}{\ensuremath{\Pi_{\textrm{RV-SPDZ}}}}
\newcommand{\HOMPED}{\ensuremath{\Pi_{\textrm{HomPed}}}}
\newcommand{\StarSS}{\ensuremath{\Pi_{\textrm{Star-SS}}}}
\newcommand{\IVMPC}{\ensuremath{\Pi_{\textrm{RV-MPC}}}}
\newcommand{\CESS}{\ensuremath{\Pi_{\textrm{CESS}}}}
\newcommand{\RCESS}{\ensuremath{\Pi_{\textrm{R-CESS}}}}
\newcommand{\RVCESS}{\ensuremath{\Pi_{\textrm{RV-CESS}}}}
\newcommand{\CatchSPDZ}{\ensuremath{\Pi_{\textrm{Catch-SPDZ}}}}

\newcommand{\com}[1][\relax]{\ensuremath{\mathsf{com}_{#1}}\xspace}
% \newcommand{\msg}[\relax]{\ensuremath{\mathit{msg}}\xspace}
\newcommand{\msg}{\ensuremath{\mathit{msg}}\xspace}
\newcommand{\Queries}{\ensuremath{\mathsf{Ans}}\xspace}
\newcommand{\notAsked}{\ensuremath{\mathsf{notAsked}}\xspace}
\newcommand{\Asked}{\ensuremath{\mathsf{Asked}}\xspace}
\newcommand{\Prove}{\ensuremath{\mathsf{Prove}}\xspace}
\newcommand{\Verify}{\ensuremath{\mathsf{Verify}}\xspace}
\newcommand{\Setup}{\ensuremath{\mathsf{Setup}}\xspace}
\newcommand{\Steps}{\ensuremath{\mathsf{Steps}}\xspace}
\newcommand{\pre}{\ensuremath{\mathsf{pre}}\xspace}
\newcommand{\Dom}{\ensuremath{\mathsf{Dom}}\xspace}
% \newcommand{\chain}{\ensuremath{\mathsf{chain}}\xspace}
\newcommand{\ver}{\ensuremath{\mathsf{ver}}\xspace}
\newcommand{\Exp}{\ensuremath{\mathsf{Exp}}\xspace}
\newcommand{\RO}{\ensuremath{\cal R}\xspace}
\newcommand{\PO}{\ensuremath{\cal P}\xspace}
%\newcommand{\R}{\ensuremath{\cal R}\xspace}
\newcommand{\Fam}{\ensuremath{\cal F}\xspace}
\newcommand{\true}{\ensuremath{\mathsf{true}}\xspace}
\newcommand{\false}{\ensuremath{\mathsf{false}}\xspace}
\newcommand{\dec}[1][\relax]{\ensuremath{\mathsf{dec}_{#1}}\xspace}
\newcommand{\skey}[1][\relax]{\ensuremath{\mathsf{sk}_{#1}}\xspace}
\newcommand{\pkey}[1][\relax]{\ensuremath{\mathsf{pk}_{#1}}\xspace}
\newcommand{\ok}{\ensuremath{\mathsf{ok}}\xspace}
\newcommand{\nok}{\ensuremath{\mathsf{nok}}\xspace}
\newcommand{\CA}{\ensuremath{\mathcal{L}_A}\xspace}

\newcommand{\cancel}[1]{}
\newcommand{\prp}{\ensuremath{{\tt ProbRelease}}\xspace}
\newcommand{\pitwo}{\ensuremath{{\tt \Pi}_2}\xspace}
%\newcommand{\pitwosfe}{\ensuremath{{\tt \pi}_{2SFE}}\xspace}
\newcommand{\pitwosfe}{\ensuremath{{\tt \Pi}_{\tt Op-SFE}}\xspace}
\newcommand{\prsfe}{\ensuremath{{\tt \Pi}_{\tt SFE}}\xspace}
%\newcommand{\prc}{\ensuremath{{\tt \pi}_{R\-2PC}}\xspace}
\newcommand{\prc}{\ensuremath{{\tt \Pi}_{\rm PFRC}}\xspace}
\newcommand{\pbot}{\ensuremath{{\tt \Pi}_\bot}\xspace}
\newcommand{\Sims}{\mathbb{S}}
%\newcommand{\Sim}{\ensuremath{\mathcal{S}}\xspace}
%\newcommand{\dummy}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\R}{\mathcal{R}}
\newcommand{\prd}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\prca}{\ensuremath{\mathcal{D_{\CA}}}\xspace}
\newcommand{\optp}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\V}{\mathcal{V}}
\newcommand{\p}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\x}{\mathcal{X}}
\newcommand{\T}{\ensuremath{\mathcal{T}}\xspace}
\newcommand{\I}{\mathcal{I}}
\newcommand{\SR}{\ensuremath{\{S,R\}}\xspace}
\newcommand{\W}{\ensuremath{\vec{W}}\xspace}
\newcommand{\SRW}{\ensuremath{\SR,\W}\xspace}
\newcommand{\doomed}{\ensuremath{\mathscr{D}}\xspace}

\newcommand{\dppu}{\ensuremath{\textsc{dppu}}\xspace}
\newcommand{\auth}{\ensuremath{\textsc{auth}}\xspace}
\newcommand{\smt}{\ensuremath{\textsc{smt}}\xspace}
\newcommand{\rauth}{\ensuremath{\textsc{r-auth}}\xspace}
\newcommand{\rsmt}{\ensuremath{\textsc{r-smt}}\xspace}
\newcommand{\Gdppu}{\ensuremath{G_{\dppu}}\xspace}
\newcommand{\smtpd}{\ensuremath{\textsc{smt-pd}}\xspace}
\newcommand{\pubsmt}{\ensuremath{\textsc{pub-smt}}\xspace}
\newcommand{\cgo}{\ensuremath{\textsc{cgo}}\xspace}
\newcommand{\upfal}{\ensuremath{\textsc{upfal}}\xspace}
\newcommand{\jrv}{\ensuremath{\textsc{jrv}}\xspace}
\newcommand{\psmt}{\ensuremath{\textsc{psmt}}\xspace}


\newcommand{\frelk}{\ensuremath{\mathcal{\frel[{\func[K07]}]}}\xspace}
%\newcommand{\pistate}{\ensuremath{\vec{\mathcal{S}}}\xspace}
\newcommand{\pistate}{\ensuremath{\vec{S}}\xspace}
\newcommand{\prel}{\bar\pi}
\newcommand{\prot}{\ensuremath{{\mathrm \Pi}}\xspace}
\newcommand{\sh}[1]{\ensuremath{\langle #1\rangle}\xspace}
\newcommand{\funsh}[1][\relax]{\ensuremath{f_{{\rm sh},#1}}\xspace}
\newcommand{\wae}{\wrap[ae]}
\newcommand{\fsh}{\func[sh]}
\newcommand{\fbc}{\func[bc]}
\newcommand{\frbc}{\func[rbc]}
\newcommand{\fsc}{\func[sc]}
\newcommand{\frc}{\func[rc]}
\newcommand{\fwc}{\func[wc]}
\newcommand{\frsc}{\func[r-sc]}
\newcommand{\fcf}[1][\relax]{\ensuremath{\func[CExch]^{#1}}\xspace}
%\newcommand{\ftf}{\ensuremath{{\func[2EX]}^\bot}\xspace}
\newcommand{\ftf}{\ensuremath{{{\mathcal F}_{\rm 2Ex}^\bot}}\xspace}
\newcommand{\fcom}{\func[com]}
\newcommand{\fauth}{\func[auth]}
\newcommand{\funauth}{\func[nauth]}
\newcommand{\fpow}{\func[pow]}
\newcommand{\fabort}{\ensuremath{\func^\perp}\xspace}
\newcommand{\fclock}{\func[clock]}
\newcommand{\fcsfe}[1][\relax]{\ensuremath{\func[com-sfe]^{#1}}\xspace}
\newcommand{\fsfe}[1][\relax]{\ensuremath{\func[sfe]^{#1}}\xspace}
\newcommand{\fmpc}[1][\relax]{\ensuremath{\func[mpc]^{#1}}\xspace}
\newcommand{\frelsfe}[1][\relax]{\ensuremath{\frel[{\fsfe[#1]}]}\xspace}
%\newcommand{\fmpc}[1][\relax]{\ensuremath{\func[rc]^{#1}}\xspace}
\newcommand{\fsfeNF}[1]{\fsfe[\bot,#1]}
\newcommand{\fsmt}{\func[smt]}
\newcommand{\frmt}{\func[rmt]}
\newcommand{\frel}[1][\ensuremath{\mathcal{F}}]{\ensuremath{\langle #1 \rangle}\xspace}
\newcommand{\fdist}{\func[rr]^{\recon}}
\newcommand{\fid}{\ensuremath{f_{\sf swp}}\xspace}
\newcommand{\vsm}[1]{\ensuremath{\tilde{#1}}\xspace}
\newcommand{\vsmset}[1]{\ensuremath{\{\cup\vsm{#1}\}}\xspace}

\newcommand{\vectorx}{\ensuremath{\mathbf x}}
\newcommand{\vectorl}{\ensuremath{\mathbf l}}
\newcommand{\Tsig}{\ensuremath{\mathsf {TSig}}}
\newcommand{\Txgen}{\ensuremath{\mathsf {Txgen}}}


\newcommand{\selParty}{\mathsf{sel}}
\newcommand{\rnd}{\mathsf{rnd}}
\newcommand{\paths}{\mathsf{paths}}
\newcommand{\aux}{\mathsf{aux}}
\newcommand{\poly}{\mathsf{poly}}
\newcommand{\sharegen}{\textnormal{\textsf{ShareGen}}}

\newcommand{\rrProt}[1][\relax]{{\mathrm \Pi}_\textsc{rr}^{#1}}
\newcommand{\btcPi}{{\mathrm \Pi}_{\sf PL}}
\newcommand{\realbtcPi}{{\mathrm \Pi}_{\sf BTC}}
\newcommand{\nakPi}{{\mathrm \Pi}_{\sf BA}^{\sf nak}}

\newcommand{\set}[1]{\mathcal{#1}}
\newcommand{\HO}{\set{H}}
\newcommand{\PS}{\ensuremath{\set{P}}\xspace}
\newcommand{\F}{\ensuremath{\mathbb{F}}\xspace}

\newcommand{\ratio}{\varrho}
\newcommand{\round}{l}
\newcommand{\rdist}{\mathcal{D}}


\newcommand{\etwopc}[1]{\ensuremath{E_{#1}^{\rm R}}\xspace}
\newcommand{\empc}[1]{\ensuremath{E_{#1}^{\rm MPC}}\xspace}


\newcommand{\erel}[1]{\ensuremath{E_{#1}^{\tt Real}}\xspace}

\newcommand{\etwopcl}[1]{\ensuremath{E_{#1}^{\tt R,\lambda}}\xspace}

\newcommand{\etwopclr}[1]{\ensuremath{E_{#1}^{\tt R,\lambda,\rho}}\xspace}

\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\diff}{d}
\newcommand{\reals}{\mathbb{R}}

\newcommand{\coloneqq}{\mathrel:\joinrel=}
\newcommand{\assign}{\coloneqq}
\newcommand{\dotcup}{\accentset{\cdot}{\cup}}
\newcommand{\natint}{\mathbf{N}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\vcom}{\ensuremath{{\tt Com}}}
\newcommand{\vdec}{\ensuremath{{\tt Dec}}}



\newcommand{\cmd}[1]{\ensuremath{\textnormal{\texttt{#1}}}\xspace}
\newcommand{\vabort}{\cmd{abort}}
\newcommand{\vactivated}{\cmd{activated}}
\newcommand{\vcorrupt}{\cmd{corrupt}}
\newcommand{\vearly}{\cmd{early}}
\newcommand{\vinput}{\cmd{input}}
\newcommand{\voutput}{\cmd{output}}
\newcommand{\vpartial}{\cmd{partial}}
\newcommand{\vready}{\cmd{ready}}
\newcommand{\pgain}[1]{\ensuremath{\textsc{Prot-Gain}_{#1}}}
\newcommand{\degfair}[1]{\ensuremath{\textsc{Deg-Fair}_{#1}}}

\newcommand{\furnd}{\ensuremath{Rnd}\xspace}
%\newcommand{\again{\texttt{rscore}}\xspace}
%\newcommand{\realscoretxt}{\ensuremath{\textnormal{\textsf{rscore}}}}
\newcommand{\realscoretxt}[1][\relax]{\ensuremath{{U^{#1}}}}
%\newcommand{\realscoretxt}[1][\relax]{\ensuremath{{U_R^{#1}}}}
\newcommand{\idealscoretxt}[1][\relax]{\ensuremath{{U^{#1}_I}}}
\newcommand{\realscorefairtxt}{\ensuremath{\textnormal{\textsf{rscore}}_{\textnormal{\textrm{fair}}}}}
\newcommand{\idealscorefairtxt}{\ensuremath{\textnormal{\textsf{iscore}}_{\textnormal{\textrm{fair}}}}}
\newcommand{\rscore}[1][\relax]{
\def\ArgRscoreI{{#1}}
\RscoreRelay
}%

% \newcommand\RscoreRelay[1][\relax]{%
% \ensuremath{%
%   \realscoretxt^{\ArgRscoreI}%
%   \ifthenelse{\equal{\relax}{#1}}{\relax}{(#1)}%
% }\xspace%
% }

\newcommand\RscoreRelay[1][\relax]{%
\ensuremath{%
    \realscoretxt[\ArgRscoreI]%
    \ifthenelse{\equal{\relax}{#1}}{\relax}{(#1)}%
}\xspace%
}


\newcommand\IscoreRelay[1][\relax]{%
\ensuremath{%
    \idealscoretxt[\ArgIscoreI]%
    \ifthenelse{\equal{\relax}{#1}}{\relax}{(#1)}}\xspace%
}

\newcommand{\rgain}{\ensuremath{\textsc{RealGain}}\xspace}
\newcommand{\iscore}[1][\relax]{
\def\ArgIscoreI{{#1}}
\IscoreRelay
}%

%\newcommand{\mgain}[2][\relax]{\ensuremath{\texttt{iscore}_{#1}^{#2}}\xspace}


\newcommand{\iscorefair}[1][\relax]{
\def\ArgIscoreIfair{{#1}}
\IscorefairRelay
}%
\newcommand\IscorefairRelay[1][\relax]{\ensuremath{\idealscorefairtxt^{\ArgIscoreIfair}(#1)}\xspace}%

\newcommand{\rscorefair}[1][\relax]{
\def\ArgRscoreRfair{{#1}}
\RscorefairRelay
}%
\newcommand\RscorefairRelay[1][\relax]{\ensuremath{\realscorefairtxt^{\ArgRscoreRfair}(#1)}\xspace}%


%\newcommand{\gaintxt}{\ensuremath{\textnormal{\texttt{gain}}}}
%\newcommand{\gaintxt}[1][\relax]{\ensuremath{\hat{U}_R^{#1}}}
\newcommand{\gaintxt}[1][\relax]{\ensuremath{\hat{U}^{#1}}}
\newcommand{\gain}[1][\relax]{
\def\ArgGainI{{#1}}
\GainRelay
}%
\newcommand\GainRelay[1][\relax]{
\ensuremath{\gaintxt[\ArgGainI](#1)}\xspace
}




%\newcommand{\gaingentxt}[1][\prot,\frel]{\ensuremath{\hat{U}_R^{#1}}}
\newcommand{\gaingentxt}[1][\prot,\frel]{\ensuremath{\hat{U}^{#1}}}

\newcommand{\gaingen}[1][\relax]{
\def\ArgGainGenI{{#1}}
\GainGenRelay
}%
\newcommand\GainGenRelay[1][\relax]{
\ifthenelse{\equal{#1}{\relax}}{%
\ensuremath{\gaingentxt[\ArgGainGenI]}
}{%
\ensuremath{\gaingentxt[\ArgGainGenI](#1)}%
}%
\xspace
}

\newcommand{\fcmax}{\ensuremath{f_{\mathrm{max}}}\xspace}
\newcommand{\fgain}[1][\func]{\ensuremath{\textsc{Gain}^{#1}}\xspace}
\newcommand{\mingain}{\ensuremath{{\tt min}\textsc{Gain}}\xspace}
\newcommand{\mfgain}{\ensuremath{\textsc{Gain}^{{\func[SFE]^{\perp}},\vec\gamma}}\xspace}
%\newcommand{\score}{\ensuremath{\textsc{x}}\xspace}
\newcommand{\score}{\ensuremath{v}\xspace}
\newcommand{\utility}{\ensuremath{u}\xspace}
%\newcommand{\score}{X}
\newcommand{\C}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\attacker}{\ensuremath{{\tt A}}\xspace}
\newcommand{\ug}{\ensuremath{u^{\G}}\xspace}
\newcommand{\designer}{\ensuremath{{\tt D}}\xspace}
%\newcommand{\G}{\ensuremath{\mathcal{G}}\xspace}
%\newcommand{\negl}{\ensuremath{\lambda}\xspace}
\newcommand{\negl}{\ensuremath{\mathsf{negl}}}
\newcommand{\id}{\ensuremath{\mathsf{id}}}
\newcommand{\noti}{\ensuremath{\mu}\xspace}
\newcommand{\itm}{\ensuremath{\mathtt{ITM}}\xspace}
%\newcommand{\iview}{\ensuremath{\mathbb{V}\textsc{iew}}}
\newcommand{\iview}{\ensuremath{\mathbb{V}}}
%\newcommand{\iview}{\ensuremath{\textsc{view}}}
\newcommand{\vcommand}[1]{\cmd{#1}}
\newcommand{\dr}{\ensuremath{\tt DummyRound}\xspace}
\newcommand{\cH}{\mathcal{H}}

\newcommand{\commit}{\mathtt{commit}}
\newcommand{\open}{\mathtt{open}}
\newcommand{\keygen}{\mathtt{keygen}}
\newcommand{\sign}{\mathtt{sign}}
\newcommand{\verify}{\mathtt{verify}}

%\DeclareMathOperator{\gain}{\textsc{gain}}

\newcommand{\mactag}{\mathsf{tag}}
\newcommand{\share}{\mathsf{share}}
\newcommand{\recon}{\mathsf{rec}}


\newcommand{\cR}{\mathcal{R}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}

% Some universal parameters
\newcommand{\parties}{n}
\newcommand{\secpar}{k}
\newcommand{\rounds}{r}
\newcommand{\random}{R}

\newcommand{\shareset}{S}

\newcommand{\grel}{\langle\mathcal{G}\rangle}
\newcommand{\hrel}{\langle\cH\rangle}

\newcommand{\ith}[1][i]{$#1$-th\xspace}

%\newcommand{\exec}{\textsc{exec}}
%\newcommand{\real}{\textsc{real}}



%\ifFull{
	
\newtheorem{lemma}{Lemma}
%\newreptheorem{lemma}{Lemma}
%\newtheorem{corollary}[lemma]{Corollary}
%\newreptheorem{corollary}{Corollary}
\newtheorem{theorem}{Theorem}
%\newreptheorem{theorem}{Theorem}
\newtheorem{claim}{Claim}
%\theoremstyle{definition}
%\newtheorem{definition}[lemma]{Definition}
%\newtheorem{example}{Example}



%\newtheorem{proposition}[lemma]{Proposition}
%\theoremstyle{remark}
%\newtheorem{remark}{Remark}


%\newtheorem{observation}[lemma]{Observation}
%}
\newtheorem{fact}{Fact}

\newenvironment{claim2}[1]{\par\noindent\emph{Claim:}\space#1}{}
\newenvironment{theorem2}[1]{\par\noindent\emph{Theorem:}\space#1}{}
\newenvironment{proofof}[1]{\par\noindent\emph{Proof:}\space#1}{\hfill $\blacksquare$}
\newenvironment{proofsketch}[1]{\par\noindent\emph{Proof sketch:}\space#1}{\hfill $\blacksquare$}



% NEW LISTS---------------------------------------------------------------

\newlength{\saveparindent}
\setlength{\saveparindent}{\parindent}
\newlength{\saveparskip}
\setlength{\saveparskip}{\parskip}


\newcounter{ctr}
\newcounter{savectr}
\newcounter{ectr}

\newenvironment{tiret}{%
\begin{list}{\hspace{1pt}\rule[0.5ex]{6pt}{1pt}\hfill}{\labelwidth=15pt%
\labelsep=3pt \leftmargin=18pt \topsep=1pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{1pt}}}{\end{list}}


\newenvironment{newenum}{%
\begin{list}{{\rm \arabic{ctr}.}\hfill}{\usecounter{ctr}\labelwidth=17pt%
\labelsep=6pt \leftmargin=23pt \topsep=.5pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{5pt} }}{\end{list}}

\newenvironment{neweenum}{%
\begin{list}{{\rm \arabic{ctr}.\arabic{ectr}}\hfill}{\usecounter{ectr}%
\labelwidth=28pt\labelsep=4pt \leftmargin=34pt \topsep=0pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{2pt} }}{\end{list}}

\newenvironment{parenum}{%
\begin{list}{{\rm (\arabic{ctr})}\hfill}{\usecounter{ctr}\labelwidth=17pt%
\labelsep=6pt \leftmargin=23pt \topsep=.5pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{5pt} }}{\end{list}}




\newenvironment{venum}{
\begin{list}{{\rm \arabic{ctr}.}\hfill}{\usecounter{ctr}\labelwidth=17pt%
\labelsep=6pt \leftmargin=23pt \topsep=.5pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{1pt} }}{\end{list}}





\newcommand{\labl}[1]{\textnormal{\textsf{#1}}}

\newcommand{\EvCorr}{\ensuremath{E_\labl{co}}\xspace}
\newcommand{\EvPriv}{\ensuremath{E_\labl{pr}}\xspace}
\newcommand{\EvCrpt}[1][\relax]{E_\labl{cp}^{#1}}

\newcommand{\payCorr}{\ensuremath{\gamma_\labl{co}}\xspace}
\newcommand{\payPriv}{\ensuremath{\gamma_\labl{pr}}\xspace}
\newcommand{\payCrpt}[1][\relax]{\ensuremath{\gamma_\labl{cp}^{#1}}\xspace}

\newcommand{\gmw}[1][\relax]{\ensuremath{\Pi_{\text{GMW}}^{#1}}\xspace}
\newcommand{\cfgn}[1][\relax]{\ensuremath{\Pi_{\text{CFGN}}^{#1}}\xspace}
\newcommand{\iklp}[1][\relax]{\ensuremath{\Pi_{\text{IKLP}}^{#1}}\xspace}
\newcommand{\psfe}[1][\relax]{\ensuremath{\Pi_{\text{Ad-SFE}}^{#1}}\xspace}
\newcommand{\ssfe}[1][\relax]{\ensuremath{\Pi_{\text{St-SFE}}^{#1}}\xspace}
\newcommand{\scoregamma}{\ensuremath{\score^{\vec\gamma}}\xspace}
\newcommand{\vrest}[2]{\ensuremath{#1|_{#2}}\xspace}

%\def\pibaoh{\Pi_{\mathsf{BA}[\sfrac{1}{2}]}}
\def\pibaoh{{\mathrm \Pi}_{\mathsf{BA}}^{\sfrac{1}{2}}}
%\def\pibaot{\Pi_{\mathsf{BA}[\sfrac{1}{3}]}}
\def\pibaot{{\mathrm \Pi}_{\mathsf{BA}}^{\sfrac{1}{3}}}
\def\powtx{{\mathrm \Pi}_{\mathsf{tx}}}

\def\tx{\mathrm{tx}}
\def\nonce{\mathit{nonce}}
\def\double-pow{\sf double-pow}




%\newcommand{\POW}{{\tt POW}\xspace}
\newcommand{\POW}{{\sf POW}\xspace}
\newcommand{\BPOW}{{\tt BPOW}\xspace}









%UC related

\newcommand{\sid}{\param{sid}}
\newcommand{\pid}{\param{pid}}
\newcommand{\xmath}[1]{\ensuremath{#1}\xspace}
\newcommand{\instr}[1]{\xmath{\textsc{#1}}}
\newcommand{\param}[1]{\xmath{\textsf{#1}}}

%Functionalities
\newcommand{\Func}[1][\relax]{\ensuremath{\mathcal{F}_{\mathsf{#1}}}\xspace}
\newcommand{\IdealFunc}[2][\relax]{\ensuremath{\mathcal{F}_{\mathsf{#1}}^{#2}}\xspace}
%$\Pi_{\textrm{OFFLINE}}$
\newcommand{\Protocol}[1][\relax]{\ensuremath{\Pi_{\textrm{OFFLINE}}}\xspace}
\iffalse
\NewDocumentCommand{\Func}{o}{%
  \ensuremath{\mathcal{F}_{%
    \IfValueTF{#1}{\textnormal{\MakeTextUppercase{\protect\unskip #1}}}{\textnormal{default}}}}%
  \xspace%
}
\fi
%\newcommand{\Func}[1][\relax]{\xmath{\mathcal{F}_{\textsc{#1}}}}
\newcommand{\wFunc}[1][\relax]{\xmath{\mathcal{W}_{\textsc{#1}}}}
\newcommand{\gFunc}[1][\relax]{\xmath{\bar{\mathcal{G}}_{\textsc{#1}}}}
\newcommand{\ggFunc}[1][\relax]{\xmath{\mathcal{G}_{\textsc{#1}}}}
\newcommand{\Simul}[1][\relax]{\xmath{\mathcal{S}_{\textsc{#1}}}}


%Registration 
\newcommand{\Register}{\instr{register}} %used by network, RO, ledger
\newcommand{\Deregister}{\instr{de-register}} %used by network, RO, ledger
\newcommand{\ARegister}{\instr{get-registered}}
\newcommand{\AFRegister}{\instr{get-registered-f}}



%-------------------------------------------------------------------------------
%  clock functionality
%-------------------------------------------------------------------------------
\newcommand{\gFclock}{\gFunc[clock]}
\newcommand{\Fclock}{\ggFunc[clock]}

\newcommand{\sidClock}{\sid_C}
\newcommand{\current}{\xmath{\tau}}
\newcommand{\ClockUp}{\instr{clock-update}}
\newcommand{\ClockRead}{\instr{clock-read}}




%-------------------------------------------------------------------------------
%  wrapper functionality
%-------------------------------------------------------------------------------
\newcommand{\Wres}{\wFunc[flt]}
\newcommand{\Wresl}{\wFunc[flt-lim]}
\newcommand{\Wleak}{\wFunc[fetch]}
\newcommand{\Wro}{\wFunc[ro]}

\newcommand{\Eval}{\instr{eval}}
\newcommand{\Failed}{\instr{fail}}
\newcommand{\Success}{\instr{success}}
\newcommand{\Continue}{\instr{continue}}
\newcommand{\Seen}{\instr{already seen}}
\newcommand{\LeakDelivery}{\instr{is-delivered}}
\newcommand{\LeakFetch}{\instr{fetch-requests}}
\newcommand{\SetRec}{\instr{set-receipts}}


%-------------------------------------------------------------------------------
%  signature functionality
%-------------------------------------------------------------------------------
\newcommand{\Fsig}{\Func[sig]}
\newcommand{\Fkes}{\Func[kes]}

\newcommand{\KGen}{\instr{KeyGen}}
\newcommand{\VKey}{\instr{Verification Key}}
\newcommand{\Sign}{\instr{Sign}}
\newcommand{\Signed}{\instr{Signed}}
\newcommand{\NotSigned}{\instr{Not Signed}}
\newcommand{\Ver}{\instr{Verify}}
\newcommand{\Vered}{\instr{Verified}}

%-------------------------------------------------------------------------------
%  registration functionality
%-------------------------------------------------------------------------------
\newcommand{\Freg}{\Func[reg]}
\newcommand{\Fsfe}{\Func[sfe]}
\newcommand{\Fcert}{\Func[a\mhyphen cert]}
\newcommand{\Fmpc}{\IdealFunc[MPC]{f}}
\newcommand{\Fampc}{\Func[A\text{-}MPC]}
\newcommand{\Favmpc}{\Func[AV\text{-}MPC]}
\newcommand{\Fcidampc}{\IdealFunc[CIDA\text{-}MPC]{f}}
\newcommand{\Fcidarmpc}{\IdealFunc[CIDA\text{-}R\text{-}MPC]{f}}
\newcommand{\Fcidarvmpc}{\IdealFunc[CIDA\text{-}RV\text{-}MPC]{f}}
\newcommand{\Frvmpc}{\IdealFunc[RV\text{-}MPC]{f}}
\newcommand{\KReg}{\instr{Submit}}
\newcommand{\KRet}{\instr{Retrieve}}
\newcommand{\Ok}{\instr{Ok}}

%  channel functionality
%-------------------------------------------------------------------------------
\newcommand{\Fauth}{\Func[auth]}
\newcommand{\FauthBD}{\Func[auth-BD]}
\newcommand{\Funfair}{\Func[m-ubc]}
\newcommand{\Fsec}{\Func[sc]}


\newcommand{\Send}{\instr{send}}
\newcommand{\Sent}{\instr{sent}}
\newcommand{\Resend}{\instr{resend}}
\newcommand{\Fetch}{\instr{fetch}}
\newcommand{\Read}{\instr{Read}}
\newcommand{\RoundOK}{\instr{Maintain}}
\newcommand{\Delay}{\instr{delay}}
\newcommand{\DelaySet}{\instr{delay set}}
\newcommand{\Replace}{\instr{replace}}
\newcommand{\Corrupted}{\instr{corrupted}}
\newcommand{\Yes}{\instr{yes}}
\newcommand{\No}{\instr{no}}
\newcommand{\predict}{\textsf{predict-time} }


%-------------------------------------------------------------------------------
%  protocols
%-------------------------------------------------------------------------------
\newcommand{\protocolone}{\texttt{Wrapped-Channel}}
\newcommand{\protocoltwo}{\texttt{Graded-Agreement}}
\newcommand{\protocolthree}{\texttt{Wrapped-Channel-Lim}}




%-------------------------------------------------------------------------------
%  oracle functionality
%-------------------------------------------------------------------------------
\newcommand{\Foracle}{\Func[\tiny{\textrm{RO}}]}

\newcommand{\ROeval}{\instr{Eval}}
\newcommand{\corrupt}{\instr{corrupt}}


%-------------------------------------------------------------------------------
%  CRS functionality
%-------------------------------------------------------------------------------
\newcommand{\Fcr}{\Func[crs]}
\newcommand{\Fcrp}{\Func[\textrm{cr-priv}]}
\newcommand{\Fcrf}{\Func[\textrm{cr-fresh}]}

\newcommand{\Wfresh}{\wFunc[fresh]}








%-------------------------------------------------------------------------------
%  Simulator Wrapped Channel
%-------------------------------------------------------------------------------
\newcommand{\SWauth}{\Simul[1]}
\newcommand{\Sreg}{\Simul[2]}

\newcommand{\CollEr}{\instr{Collision-Error}}
\newcommand{\PRO}{{\cal P}_{RO}}
\newcommand{\PNET}{{\cal P}_{Net}}
\newcommand{\PADV}{\tilde{{\cal P}}}









%%%%%%%%  Boxes %%%%%%%%%%%%%



%-------------------------------------------------------------------------------
%  Magic Stuff below
%-------------------------------------------------------------------------------

%------ Quote ---------------------------------------------------------------

\renewcommand{\quote}{\list{}{\rightmargin=\leftmargin\topsep=0pt}\item\relax}

%------ Subsection and Paragraph --------------------------------------------

\makeatletter
%\renewcommand{\section}{\abovedisplayskip 3\p@ \@plus3\p@ \@minus1\p@%
%                      \belowdisplayskip 5\p@ \@plus3\p@ \@minus1\p@%
%                      \abovedisplayshortskip 0pt \@plus2\p@%
%                      \belowdisplayshortskip 0pt \@plus2\p@ \@minus0\p@%
%                      \@startsection{section}{1}{\z@}%
%                       {-10\p@ \@plus -4\p@ \@minus -4\p@}%
%                       {6\p@ \@plus 4\p@ \@minus 4\p@}%
%                       {\normalfont\large\bfseries\boldmath
%                        \rightskip=\z@ \@plus 8em\pretolerance=10000 }}
%\renewcommand{\subsection}{\@startsection{subsection}{2}{\z@}%
%                      {-6\p@ \@plus -4\p@ \@minus -4\p@}%
%                      {2\p@ \@plus 2\p@ \@minus 2\p@}%
%                      {\normalfont\normalsize\bfseries\boldmath
%                       \rightskip=\z@ \@plus 8em\pretolerance=10000 }}
\renewcommand{\subsubsection}{\@startsection{paragraph}{4}{\z@}%
	{-8\p@ \@plus -4\p@ \@minus -4\p@}%
	{-5\p@ \@plus -0.22em \@minus -0.1em}%
	{\normalfont\normalsize\bfseries\boldmath
	}}
\renewcommand{\paragraph}{\@startsection{paragraph}{4}{\z@}%
	{-8\p@ \@plus -4\p@ \@minus -4\p@}%
	{-5\p@ \@plus -0.22em \@minus -0.1em}%
	{\normalfont\normalsize\em
	}}
	\makeatother
	

	
%----- Comments ----------------------------------------------------------------
\definecolor{lightgreen}{rgb}{0.86, 0.93, 0.78}
\definecolor{bordergreen}{rgb}{0.55, 0.76, 0.74}
\definecolor{lightblue}{rgb}{0.70, 0.90, 0.99}
\definecolor{borderblue}{rgb}{0.01, 0.66, 0.96}
\definecolor{lightamber}{rgb}{1, 0.93, 0.70}
\definecolor{borderamber}{rgb}{1, 0.76, 0.03}

%----- Algorithm Environment ---------------------------------------------------
%Header for Algorithms/Functionalities
\newcommand{\algoHead}[1]{\vspace{0.2em} \underline{\textbf{#1}} \vspace{0.3em}}
\newcommand{\algoHeadExt}[2]{\vspace{0.2em} \underline{\textbf{#1} #2} \vspace{0.3em}}

%Multiline Algo-States
\makeatletter
\algnewcommand{\ExtendedState}[1]{\State
	\parbox[t]{\dimexpr\linewidth-\ALG@thistlm}{\hangindent=\algorithmicindent\strut\hangafter=3#1\strut}}
\makeatother

%Algorithms States
\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

%Algo Comments
\algrenewcommand{\algorithmiccomment}[1]{{\color{gray}// #1}}

%----- Box Environment ---------------------------------------------------------
\RequirePackage{mdframed}

%Basic box structure with title box
\newenvironment{titlebox}[3]
{\mdfsetup{
		style=#2,
		innertopmargin=1.1\baselineskip,
		skipabove={\dimexpr0.7\baselineskip+\topskip\relax},
		skipbelow={1em},needspace=3\baselineskip,
		singleextra={\node[#3,right=10pt,overlay] at (P-|O){~{\sffamily\bfseries #1 }};},%
		firstextra={\node[#3,right=10pt,overlay] at (P-|O) {~{\sffamily\bfseries #1 }};},
		frametitleaboveskip=9em,
		innerrightmargin=5pt
	}
	\begin{mdframed}[font=\small]\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}	\raggedright% 
	}
	{\end{mdframed}}

%title box style
\tikzstyle{normal} = [thick, fill=white, text=black, draw, rounded corners, rectangle, minimum height=.7cm, inner sep=3pt]
\tikzstyle{gray} = [thick, fill=gray!90, text=white, rounded corners, rectangle, minimum height=.7cm, inner sep=3pt]

%box style
\mdfdefinestyle{commonbox}{%
	align=center, middlelinewidth=1.1pt,userdefinedwidth=\linewidth
	innerrightmargin=0pt,innerleftmargin=5pt,innertopmargin=5pt,
	splittopskip=15pt,splitbottomskip=15pt
}
\mdfdefinestyle{roundbox}{style=commonbox,roundcorner=5pt,userdefinedwidth=\linewidth}

\newenvironment{systembox}[1]
{\vspace{\baselineskip}\begin{titlebox}{Functionality \normalfont #1}{roundbox}{normal}}
	{\end{titlebox}}

\newenvironment{wsystembox}[1]
{\vspace{\baselineskip}\begin{titlebox}{Wrapper Functionality \normalfont #1}{roundbox}{normal}}
	{\end{titlebox}}

\newenvironment{gsystembox}[1]
{\vspace{\baselineskip}\begin{titlebox}{Global Functionality \normalfont #1}{roundbox}{normal}}
	{\end{titlebox}}

\newenvironment{protocolbox}[1]
{\begin{titlebox}{{\bf Protocol} \normalfont #1}{commonbox}{normal}}
	{\end{titlebox}}

\newenvironment{algobox}[1]
{\begin{titlebox}{Algorithm \normalfont #1}{commonbox}{normal}}
	{\end{titlebox}}

\newenvironment{reductionbox}[1]
{\begin{titlebox}{Reduction \normalfont #1}{commonbox}{normal}}
	{\end{titlebox}}

\newenvironment{gamebox}[1]
{\begin{titlebox}{Game \normalfont #1}{commonbox}{gray}}
	{\end{titlebox}}

\newenvironment{simulatorbox}[1]
{\begin{titlebox}{Simulator \normalfont #1}{commonbox}{normal}}
	{\end{titlebox}}

%----- Old macros --------------------------------------------------------------
%For old macros
\newcommand{\deprecated}[1][\relax]{%
	\begin{tikzpicture}[baseline=(A.south)]
	\node (A) [] at (0,0){};
	\node [rectangle, draw, fill=red!20,text=black](B) at (0.1ex,0ex){
		\raggedright DO NOT USE! 
		\if #1\relax\else
		Use instead: #1
		\fi
	};
	\end{tikzpicture}
}


